A Novel Nonlinear Nonparametric Correlation Measurement With A Case Study on Surface Roughness in Finish Turning

Estimating the correlation coefficient has been a daunting work with the increasing complexity of dataset's pattern. One of the problems in manufacturing applications consists of the estimation of a critical process variable during a machining operation from directly measurable process variables. For example, the prediction of surface roughness of a workpiece during finish turning processes. In this paper, we did exhaustive study on the existing popular correlation coefficients: Pearson correlation coefficient, Spearman's rank correlation coefficient, Kendall's Tau correlation coefficient, Fechner correlation coefficient, and Nonlinear correlation coefficient. However, no one of them can capture all the nonlinear and linear correlations. So, we represent a universal non-linear non-parametric correlation measurement, g-correlation coefficient. Unlike other correlation measurements, g-correlation doesn't require assumptions and pick the dominating patterns of the dataset after examining all the major patterns no matter it is linear or nonlinear. Results of testing on both linearly correlated and non-linearly correlated dataset and comparison with the introduced correlation coefficients in literature show that g-correlation is robust on all the linearly correlated dataset and outperforms for some non-linearly correlated dataset. Results of the application of different correlation concepts to surface roughness assessment show that g-correlation has a central role among all standard concepts of correlation.

==> bib.tex <==
@misc{fleming1994principles,
  title={Principles of Applied Statistics Rout ledge, London National Guidelines and standards for industrial Effluents, Gaseous, Emissions and hazardous waste Management in Nigeria},
  author={Fleming, Michael C and others},
  year={1994},
  publisher={FEP}
}

@book{richards1998zen,
  title={The Zen of empirical research},
  author={Richards, William D},
  year={1998},
  publisher={Hampton Press}
}

@misc{pfeifferprobability,
  title={Probability for Applications. 1990},
  author={Pfeiffer, PE},
  publisher={Springer-Verlag}
}

@article{hogg1997sampling,
  title={Sampling distribution theory},
  author={Hogg, RV and Tanis, EA},
  journal={Probability and Statistical Inference. Prentice-Hall, Upper Saddle River, NJ},
  pages={262--3},
  year={1997}
}

@article{drake1996assessment,
  title={Assessment of solar and wind energy resources in Ethiopia. I. Solar energy},
  author={Drake, Frances and Mulugetta, Yacob},
  journal={Solar energy},
  volume={57},
  number={3},
  pages={205--217},
  year={1996},
  publisher={Elsevier}
}

@article{rohatgi1976introduction,
  title={An Introduction to Probability Theory and Mathematical Statistics. Ed. John Wiley \& Sons},
  author={Rohatgi, VK},
  year={1976}
}

@article{hollander1999nonparametric,
  title={Nonparametric statistical methods},
  author={Hollander, Myles and Wolfe, Douglas A},
  year={1999},
  publisher={Wiley-Interscience}
}

@book{freeman1965elementary,
  title={Elementary applied statistics: for students in behavioral science},
  author={Freeman, Linton C},
  year={1965},
  publisher={John Wiley \& Sons}
}

@misc{hartung1999statistik,
  title={Statistik-{\"U}bungen. Deskriptive Statistik. 6. Aufl. M{\"u}nchen/Wien},
  author={Hartung, Joachim and Heine, Barbara},
  year={1999},
  publisher={R. Oldenbourg}
}

@article{lindley1965introduction,
  title={Introduction to probability and statistics fom a Bayesian view point (partI and II) Cambridge University press},
  author={Lindley, DV},
  year={1965}
}

@book{sheskin2003handbook,
  title={Handbook of parametric and nonparametric statistical procedures},
  author={Sheskin, David J},
  year={2003},
  publisher={crc Press}
}

@article{pittner2000correlation,
  title={Correlation between acoustic emission statistics and surface roughness in finish turning},
  author={Pittner, Stefan and Kamarthi, Sagar V and Wongsiripatanakul, Piroj and Wongvasu, Naken},
  journal={Citeseerx Google Scholar},
  year={2000}
}

@book{wesolowsky1976multiple,
  title={Multiple regression and analysis of variance: An introduction for computer users in management and economics},
  author={Wesolowsky, George O},
  year={1976},
  publisher={John Wiley \& Sons}
}

@INPROCEEDINGS{5382400,
  author={Shen, Zhiyuan and Wang, Qiang and Shen, Yi},
  booktitle={2009 IEEE Youth Conference on Information, Computing and Telecommunication}, 
  title={A new non-liner correlation measure}, 
  year={2009},
  volume={},
  number={},
  pages={11-14},
  keywords={Mutual information;Information entropy;Data analysis;Logistics;Random variables;Testing;Statistics;Grain size;Mathematics;Information analysis;Entropy;nonlinear correlation;mutual information;correlation coefficient},
  doi={10.1109/YCICT.2009.5382400}}
@misc{Latyshev_Koldanov_1970a, title={Investigation of connections between Pearson and Fechner correlations in market network: Experimental study}, url={https://link.springer.com/chapter/10.1007/978-3-319-29608-1_12}, journal={SpringerLink}, publisher={Springer International Publishing}, author={Latyshev, Andrey and Koldanov, Petr}, year={1970}, month={Jan}} 

